New Trade-Offs for Fully Dynamic Matching via Hierarchical EDCS

We study the maximum matching problem in fully dynamic graphs: a graph is undergoing both edge insertions and deletions, and the goal is to efficiently maintain a large matching after each edge update. This problem has received considerable attention in recent years. The known algorithms naturally exhibit a trade-off between the quality of the matching maintained (i.e., the approximation ratio) and the time needed per update. While several interesting results have been obtained, the optimal behavior of this trade-off remains largely unclear. Our main contribution is a new approach to designing fully dynamic approximate matching algorithms that in a unified manner not only (essentially) recovers all previously known trade-offs that were achieved via very different techniques, but reveals some new ones as well. As our main tool to achieve this, we introduce a generalization of the edge-degree constrained subgraph (EDCS) of Bernstein and Stein (2015) that we call the hierarchical EDCS (HEDCS).

==> randEDCS.tex <==
\clearpage
\section{Randomized EDCS}

Let $G=(V, E)$ be a fully dynamic graph subject to edge insertions and deletions. We use $G_i$ to denote the graph after the $i$-th update. Upon insertion of any edge $e$ to $G$, we reveal a random rank $\pi(e) \in [0, 1]$ independently and uniformly at random.\footnote{We emphasize that the sequence of updates to $G$ is oblivious to the random ranks. That is, one can assume that the sequence of updates is fixed before any randomization is revealed.}
For any parameter $p > 0$, we use $G^p$ to denote a subgraph of $G$ including only edges $e$ of $G$ with $\pi(e) < p$. In other words, $G^p$ is a random subgraph of $G$ including each edge independently with probability $p$. We may also use $G^p_i$ to denote the subgraph of $G_i$ including only edges $e \in G_i$ with $\pi(e) < p$.

\subsection*{The Algorithm}
\newcommand{\ADD}[0]{\ensuremath{\mathsf{ADD}}}
\newcommand{\DEL}[0]{\ensuremath{\mathsf{DEL}}}


For some $\beta \geq 2$, we would like to maintain a \underline{$\beta$-EDCS} $H$ of random subgraph $G^p$ which satisfies:
\begin{enumerate}
	\item For any $e = (u, v) \in H$, $\deg_H(u) + \deg_H(v) \leq \beta$.
	\item For any $e = (u, v) \in G^p \setminus H$, $\deg_H(u) + \deg_H(v) \geq \beta - 1$.
\end{enumerate}
To do so, suppose that up to the $(i-1)$-th update, we have a $\beta$-EDCS $H_{i-1}$ of $G^p_{i-1}$. It remains to show how we address the $i$-th update. Let $e=(u, v)$ be the edge being inserted or deleted. We run Algorithm~\ref{alg:update} below to make sure $H_i$ remains to be a valid EDCS of $G^p_i$.

\begin{algorithm}[H]
	\If{$\pi(e) > p$}{\Return}
	
	\If{$e$ is being inserted and $\deg_{H_{i-1}}(u) + \deg_{H_{i-1}}(v) < \beta - 1$}{
		$H_i \gets \ADD(e, H_{i-1}, G_i^p)$.
	}
	
	\If{$e$ is being deleted and $e \in H_{i-1}$}{
		$H_i \gets \DEL(e, H_{i-1}, G_i^p)$.
	}
	
	\caption{The update algorithm for the $i$-th edge insertion/deletion of edge $e=(u, v)$.}	
	\label{alg:update}
\end{algorithm}

Subroutine $\ADD(e, H, G^p_i)$ is defined as follows:

\begin{algorithm}[H]
	$H \gets H \cup \{e\}$.
	
	Let $F_u := \{ w \in V \mid (u, w) \in H \text{ and } \deg_H(u) + \deg_H(w) > \beta \}$.
	
	\If{$F_u \not= \emptyset$}{
		Pick some $w \in F_u$ arbitrary and let $H \gets \DEL((u, w), H, G_i^p)$.
	}
	
	Let $F_v := \{ w \in V \mid (v, w) \in H \text{ and } \deg_H(v) + \deg_H(w) > \beta \}$.
	
	\If{$F_v \not= \emptyset$}{
		Pick some $w \in F_v$ arbitrary and call $H \gets \DEL((v, w), H, G_i^p)$.
	}
	\Return $H$
	
\caption{\ADD($e=(u, v), H, G_i^p$)}
\end{algorithm}

And subroutine $\DEL(e, H, G^p_i)$ is as follows:

\begin{algorithm}[H]
	$H \gets H \setminus \{e\}$.
	
	Let $U_u := \{ w \in V \mid (u, w) \in G_i^p \setminus H \text{ and } \deg_H(u) + \deg_H(w) < \beta - 1 \}$.
	
	\If{$U_u \not= \emptyset$}{
		Pick some $w \in U_u$ arbitrary and let $H \gets \ADD((u, w), H, G^p_i)$.
	}
	
	Let $U_v := \{ w \in V \mid (v, w) \in G^p_i \setminus H \text{ and } \deg_H(v) + \deg_H(w) < \beta - 1 \}$.
	
	\If{$U_v \not= \emptyset$}{
		Pick some $w \in U_v$ arbitrary and call $H \gets \ADD((v, w), H, G^p_i)$.
	}
	\Return $H$
	
\caption{\DEL($e=(u, v), H, G^p_i$)}
\end{algorithm}

\begin{claim}
	Algorithm~\ref{alg:update} changes the $H$-degree of at most $O(\beta)$ vertices with probability 1. Furthermore, the update-time of each edge insertion/deletion can be bounded by $O(p \beta \Delta)$ in expectation.\footnote{We note with a slightly smarter update algorithm that explicitly stores the edges of $G^p$ one can also achieve $O(p^2 \beta \Delta)$ expected update-time, but this will not affect our final guarantee so we prove the simpler bound here.}
\end{claim}
\begin{proof}[Proof sketch]
	Fix an edge update $e$. If $\pi(e) \geq p$ we do not do anything, so we only spend time updating the EDCS if $\pi(e) < p$ which occurs with probability $\leq p$. We show that conditioned on $\pi(e) < p$, the update time can be deterministically bounded by $O(\beta \Delta)$.
	
	To prove this deterministic bound, note that adding or removing $e$ to the EDCS causes a cascade of updates to $H$ through recursive calls to $\ADD$ and $\DEL$ subroutines. One can bound the total number of these recursive calls by $4 \beta$ (see Section~C.1 of \cite{BernsteinStein15ArXiv}). This immediately proves the part of the claim that the degrees of at most $O(\beta)$ vertices change. Furthermore, each call by itself (i.e., ignoring the cost of recursive calls) can be done in $O(\Delta)$ time as we only have to scan incident edges to the two endpoints of the edge being added/deleted. Thus, the total expected update-time can be bounded by $O(p \beta \Delta)$.
\end{proof}

\subsection{Sparsification Property}

For any $i$, define $$U_i := \{e = (u, v) \in G_i \mid \deg_{H_i}(u) + \deg_{H_i}(v) < \beta - 1\}$$ to be the set of edges in the whole graph up to the $i$-th update that are ``uncovered'' by the EDCS $H_{i}$. Note that since $H_i$ is a valid EDCS of $G^p_i$ it leaves no uncovered edge in $G^p_i$ so all the edges of $U_i$ must be in $G_i \setminus G^p_i$.

\begin{lemma}
	Fix any $i$; with probability $1-n^{-5}$ the maximum degree in $U_i$ is at most $O(p^{-1} \beta \log n)$.  
\end{lemma}

